Ask an Expert: Leveraging Language Models to Improve Strategic Reasoning in Goal-Oriented Dialogue Models

Existing dialogue models may encounter scenarios which are not well-represented in the training data, and as a result generate responses that are unnatural, inappropriate, or unhelpful. We propose the "Ask an Expert" framework in which the model is trained with access to an "expert" which it can consult at each turn. Advice is solicited via a structured dialogue with the expert, and the model is optimized to selectively utilize (or ignore) it given the context and dialogue history. In this work the expert takes the form of an LLM. We evaluate this framework in a mental health support domain, where the structure of the expert conversation is outlined by pre-specified prompts which reflect a reasoning strategy taught to practitioners in the field. Blenderbot models utilizing "Ask an Expert" show quality improvements across all expert sizes, including those with fewer parameters than the dialogue model itself. Our best model provides a $\sim 10\%$ improvement over baselines, approaching human-level scores on "engingingness" and "helpfulness" metrics.

==> tables/dialogue_auto.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{rcccc}
    \toprule
         \textbf{Model}    &  \textbf{F-1}           &  \textbf{BLEU-4}            &    \textbf{PPL$\downarrow$}   &  \textbf{token-acc} \\
         \midrule
         BB       & .190           &  .009              &    12.32             &   .448     \\
         \midrule
         BBMH     & \textbf{.553}           &  \textbf{.421}              &    \textbf{\phantom{0}1.16}   &   \textbf{.971}     \\
         \midrule
         BBMHR:   &                                    \\
\textit{GPT-1}    & .192           &  .010              &    33.52             &   .408     \\
\textit{GPT-2}    & .194           &  .013              &    30.61             &   .414     \\
\textit{ada}      & .194           &  .011              &    27.99             &   .413     \\
\textit{davinci}  & .202           &  .015              &    28.71             &   .412     \\
    \bottomrule
    \end{tabular}
    \caption{Automatic evaluation results of different models.}
    \label{tab:autoresults}
\end{table}

==> tables/distil_effectiveness.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{rcc}
    \toprule
    \textbf{Scores} & \textbf{GPT-2} & \textbf{DistilGPT-2} \\
    \midrule
    \multicolumn{3}{l}{\textit{Similarity Scores}} \\
    \midrule
    BLEU-4    & \textbf{\phantom{0}0.06}  & \phantom{0}0.01\\
    ROUGE-L   & \phantom{0}0.24  & \textbf{\phantom{0}0.26}\\
    BERTScore & \textbf{88.14} & 86.78\\
    BARTScore & - 4.41 & \textbf{- 4.33} \\
    \midrule
    \multicolumn{3}{l}{\textit{Entailment Scores}} \\
    \midrule
    RoBERTa   & 1.23  & \textbf{1.37} \\
    DeBERTa   & \textbf{0.74}  & 0.70 \\
    \bottomrule
    \end{tabular}
    \caption{Automatic evaluation on reasoning processes by GPT-2 and DistilGPT-2.}
    \label{tab:distil}
\end{table}

==> tables/error.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lc}
    \toprule
         \textbf{Model}  &  \textbf{Ignoring Rates}\\
    \midrule
         BBMHR + \textit{GPT-1} &  17.78\\
         BBMHR + \textit{GPT-2} &  16.31\\
         BBMHR + \textit{ada} &  14.13\\
         BBMHR + \textit{davinci} &  15.78\\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Ignoring rates.} Percentages of responses that ignore the reasoning annotations and do not follow the suggestion for supporters from PLMs for each BBMHR model.}
    \label{tab:not_following}
\end{table}

==> tables/out_of_content.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ccc}
    \toprule
    \textbf{Error responses} & Error responses by & \textbf{Error rates by} \\
    \textbf{Number} & incorrect reasoning  & \textbf{incorrect reasoning} \\
    \midrule
        BBMHR + GPT-1 &  00.0\\
        BBMHR + GPT-1 &  \\
        BBMHR + GPT-1 &  \\
        BBMHR + GPT-1 &  \\
    \bottomrule
    \end{tabular}
    \caption{Rates of the responses that are out of context when the PLMs return incorrect reasoning annotations or inappropriate suggestions for supporter.}
    \label{tab:out_of_context}
\end{table}
